Pricing and Hedging Basket Options with Exact Moment Matching

Theoretical models applied to option pricing should take into account the empirical characteristics of the underlying financial time series. In this paper, we show how to price basket options when assets follow a shifted log-normal process with jumps capable of accommodating negative skewness. Our technique is based on the Hermite polynomial expansion that can match exactly the first m moments of the model implied-probability distribution. This method is shown to provide superior results for basket options not only with respect to pricing but also for hedging.

==> LevyModel.tex <==
The market is described by the  $N$-dimensional
stock price process:
\begin{equation}\label{stock price process}
S_t^{(i)}=S_0^{(i)}\exp\left( (r-q_i+\omega_i)t + Y_t^{(i)}  \right),
\quad i=1,\ldots,N
\end{equation}
where
$\bm{Y}_t =(Y_t^{(1)},\ldots,Y_t^{(N)})'$
is an $N$-dimensional L\'{e}vy process,
 $r$ is the risk-free rate,
$q_i$ the dividend yield of stock $i$,
and
$\omega_i=-K_{Y_t^{(i)} }(1)/t=-K_{Y_1^{(i)} }(1)$
is the mean correcting term\footnote{Here $K_{X}(s)=\log[m_{X}(s)]$ and $m_{X}(s)=\esp[\ee^{s X}]$
are the cumulant and moment generating function of the random variable $X$, respectively.} for stock $i$ that makes
the model risk-neutral, i.e.
\begin{equation}
\esp[S_t^{(i)}]=S_0^{(i)}\exp\left( (r-q_i)t   \right),
\forall i=1,\ldots,N.
\end{equation}
The money market account $\{M_t\}_{0\leq t}$ is described by
\begin{equation}
dM_t = rM_t dt.
\end{equation}

\subsection{Moments of the Basket}
Our aim is to price basket options
under model \eqref{stock price process}.
The underlying variable is
\begin{equation}\label{basket}
B_t =\sum_{i=1}^N a_i S_t^{(i)}
\end{equation}
where $\bm{a}  =(a_1,\ldots,a_N)'$
is a vector of basket weights, positive or negative.
Under many models applied in practice the probability density of a basket $B_t$ is not known in closed form.

The methodology proposed here is focused on using a Hermite approximation probability density that will replace the risk-neutral density implied by the model~\eqref{stock price process}. The approximation density derived in this paper is constructed in such a way to match exactly up to the first six moments of the model implied risk-neutral density.

Thus, the first step in our methodology is to derive the moments of the basket~\eqref{basket} under the specification of the general model~\eqref{stock price process}.
If  $m_{\bm{Y}_t}(\bm{u})=\esp[\ee^{\bm{u}'\bm{Y}_t}]$
is the moment generation function (mgf) of vector $\bm{Y}_t$, it follows that
\begin{gather*}
\label{moments}
\mu_k = \esp[B_t^k]
=\sum_{i_1=1}^N\cdots\sum_{i_k=1}^N
\left( a_{ i_1 } S_0^{(i_1)}  \ee^{  (r-q_{i_1}+\omega_{i_1})t    }\right)\cdots
\left( a_{ i_k } S_0^{(i_k)}  \ee^{  (r-q_{i_k}+\omega_{i_k})t   }\right)\\
\times m_{\bm{Y}_t}(\bm{e}_{ i_1 } + \ldots + \bm{e}_{ i_k })
\end{gather*}
where
$\bm{e}_i$ denotes the $N\times 1$ vector
with all zeros and 1 in position $i$.
%\subsection{GBM}

For exemplification several well-known models are discussed.
\subsubsection{Multivariate Gaussian Model}
 For the case when  $S_t^{(i)}$ follow a multivariate geometric Brownian motion (GBM), it is well-known that
\begin{equation}\label{GBM mgf}
m_{\bm{Y}_t}(\bm{u})=\exp\left( t\bm{u}'\bm{\Sigma}\bm{u}/2\right)
\end{equation}
where the element in position $(i,j)$
of the covariance matrix $\bm{\Sigma}$
is $\bm{\Sigma}_{i,j}=\sigma_i\sigma_j\rho_{i,j}$.
Thus, $\omega_i=-\sigma^2_i/2$.

\subsubsection{The Variance Gamma Model}

In the case of the $\alpha$-VG Model
\begin{gather}
Y_t^{(i)}=\theta_i  G_t^{(i)} + \sigma_i W_{G_t^{(i)}} , \nonumber\\
G_t^{(i)}= X_t^{(i)} + \alpha_i Z_t, \quad i=1,\ldots,N
\end{gather}
where $W^{(i)}$ are independent standard
Brownian motions, the subordinator $G^{(i)}$
is the weighted sum of two independent
Gamma process. In particular
$X_t^{(i)}\sim \Gamma(a_it,b_i)$ so that
$m_{X_t^{(i)}}(u)=(1-u/b_i)^{(-a_i t)}$ for
$u  < b_i$ and
$Z_t  \sim \Gamma(c_1 t,c_2)$ so that
$m_{Z_t}(s)=(1-s/c_2)^{(-c_1 t)}$ for
$s  < c_2$. For this model all parameters
are required to be positive, with the exception
of $\theta_i$.

The mgf of
$\bm{Y}_t$ is
\begin{equation}\label{alphaVG mgf}
m_{\bm{Y}_t}(\bm{u})=
m_{Z_t}\left(  \bm{\alpha}'\bm{d}   \right)
\prod_{i=1}^N m_{X_t^{(i)}}(d_i)
\end{equation}
where
\begin{gather*}
\bm{\alpha} =(\alpha_1,\ldots,\alpha_N)' ,\\
\bm{d} =( d_1,\ldots, d_N)' ,\\
d_i= u_i\theta_i + \sigma_i^2 u_i^2/2
\quad i=1,\ldots,N.
\end{gather*}
Note that, in order
to ensure that the business time
increases on average as the real
time $t$ we need the additional
constraints
\[
\frac{a_i}{b_i}=1-\alpha_i\frac{c_1}{c_2},\quad i=1,\ldots,N.
\] 



==> Merton_Model_General.tex <==
\subsubsection{The General Multivariate Jump-Diffusion Model}
Consider now the case of the general multivariate jump-diffusion model given by
\begin{equation}\label{ith component sys+spec}
Y_t^{(i)}= \sigma_i   W_t^{(i)} + \sum_{h=1}^{N_t} J_h^{(\text{sys},i)}
+\sum_{h_i=1}^{N_t^{(i)}}J_{h_i}^{(\text{spec},i)}
\quad i=1,\ldots,N
\end{equation}
where
\begin{gather*}
J_h^{(\text{sys},i)}  \sim  N(\gamma_{\text{sys},i},\delta^2_{\text{sys},i})\\
J_{h_i}^{(\text{spec},i)}  \sim  N(\gamma_{\text{spec},i},\delta^2_{\text{spec},i})\\
\cov\left( J_h^{(\text{sys},i)}   ,  J_l^{(\text{sys},i)}  \right)=0 \quad\forall i=1,\ldots,N,\quad\text{and} \quad\forall h\neq l\\
\cov\left(J_h^{(\text{sys},i)},J_h^{(\text{sys},j)}\right)=\delta_{\text{sys},i}\delta_{\text{sys},j}c_{i,j} \quad\forall i,j=1,\ldots,N
\quad\text{and} \quad\forall h\\
\cov\left( J_h^{(\text{spec},i)}   ,  J_l^{(\text{spec},i)}  \right)=0 \quad\forall i=1,\ldots,N,\quad\text{and} \quad\forall h\neq l\\
\cov\left(J_h^{(\text{spec},i)},J_h^{(\text{spec},j)}\right)=0 \quad\forall i,j=1,\ldots,N
\quad\text{and} \quad\forall h\\
\cov\left( J_h^{(\text{spec},i)}   ,  J_l^{(\text{sys},j)}  \right)=0 \quad\forall i,j=1,\ldots,N,\quad\text{and} \quad\forall h, l\\
\end{gather*}
and where $\{N_t\}_{0\leq t}$ and $\{N_t^{(i)}\}_{0\leq t}$ are independent Poisson process with intensity
$\lambda_{\text{sys}}$ and $\lambda_{\text{spec},i}$, respectively.
We assume all jumps to be
independent on the Brownian motions
and on the Poisson processes. Furthermore,
the Brownian motions
and  the Poisson processes
are independent.

Denoting by $\bm{\Sigma}$
the covariance matrix of
$\bm{W}_1=(W_1^{(1)},\ldots,W_1^{(N)})'$, and
by $\bm{\Gamma}_\text{sys}$
the covariance matrix of
$\bm{J}=(J^{(\text{sys},1)},\ldots,J^{(\text{sys},N)})'$,
 the mgf of
$\bm{Y}_t$ is\footnote{
This follows from the fact that we
can write
\[
Y_t^{(i)}= \sigma_i   W_t^{(i)} +  N_t\gamma_{\text{sys},i} + \delta_{\text{sys},i}\sqrt{N_t} Z^{(i)}
+  N_t^{(i)}\gamma_{\text{spec},i}   + \delta_{\text{spec},i} \sqrt{N_t^{(i)}} Z^{(\text{spec},i)}
\quad i=1,\ldots,N
\]
with $Z^{(i)}$ and $Z^{(\text{spec},i)}$ are independent
standard normal.
Hence, conditional on $N_t$
and on the vector $\bm{N}_t=\left(N_t^{(1)},\ldots,N_t^{(N)}\right)'$
 the vector $\bm{Y}_t$
is multivariate normal with
mean $\bm{\gamma}_\text{sys} N_t + \bm{N}_t \circ \bm{\gamma}_{\text{spec}}$
and covariance $t\bm{\Sigma} + N_t\bm{\Gamma}\text{sys} + \diag( \bm{N}_t\circ \bm{\gamma}_{\text{spec}} \circ\bm{\gamma}_{\text{spec}} )$.
Here we denote by
$\bm{\gamma}_{\text{spec}}  =( \gamma_{\text{spec},1},\ldots,\gamma_{\text{spec},N})'$
and by
$\bm{\delta}_{\text{spec}}  =( \delta_{\text{spec},1},\ldots,\delta_{\text{spec},N})'$
the vectors of asset-specific jump mean
and standard deviations, respectively
and by $\circ$ the Hadamard product (i.e. entrywise product).
}
\begin{equation}\label{MultivariateMerton sys + spec mgf}
m_{\bm{Y}_t}(\bm{u})=
\exp\left( t\bm{u}'\bm{\Sigma}\bm{u}/2\right) m_{N_t}\left(  \bm{\gamma}_{\text{sys}}'\bm{u} + \bm{u}'\bm{\Gamma}_{\text{sys}}\bm{u}/2 \right)\left( \prod_{i=1}^N m_{N_t^{(i)}}(  \gamma_{\text{spec},i} u_i + \delta^2_{\text{spec},i}u_i^2/2  ) \right)
\end{equation}
where $\bm{\gamma}_{\text{sys}}  =( \gamma_{\text{sys},1},\ldots,\gamma_{\text{sys},N})'$,
$m_{N_t}(u)=\exp(t\lambda_{\text{sys}} (\ee^u-1))$,
and $m_{N_t^{(i)}}(u)=\exp(t\lambda_{\text{spec},i} (\ee^u-1))$.
For this model the mean correcting term
associated with the stock $i$ is
\begin{eqnarray}
\omega_i&=&-\sigma^2_i/2- \lambda_{\text{sys}}  k_{\text{sys},i} -\lambda_{\text{spec},i}   k_{\text{spec},i}
=\nonumber\\
&=&-\sigma^2_i/2-\lambda_{\text{sys}}(\exp(\gamma_{\text{sys},i}+\delta_{\text{sys},i}^2/2)-1)+\nonumber\\
&-&\lambda_{\text{spec},i}(\exp(\gamma_{\text{spec},i}+\delta_{\text{spec},i}^2/2)-1)
.
\end{eqnarray}


==> ResultHermiteGBM.tex <==
\subsection{Comparisons under Multi-dimensional GBM Model}
In this section a comparison among the different methods to price basket and spread options when underlying assets in the basket follows GBM. The results are in table \ref{tab:result}. %and in particular the methods compared are:
%\begin{itemize}
%\item Monte Carlo with the control variates in section \ref{controlVariates} with $10^6$ paths (in parentheses the standard deviation)
%\item standard Monte Carlo  with $10^6$ paths  (in parentheses the standard deviation)
%\item generalized log-normal distribution (Borovkova, Permana and Weide (2007))
%\item hermite tree by matching the first \textbf{four} moments of the \textbf{log-returns} of the basket
%\item hermite tree by matching the first \textbf{four}  moments of the \textbf{returns} of the basket
%\item hermite tree by matching the first \textbf{four}  moments of the \textbf{value} of the basket
%\item hermite tree by matching the first \textbf{six}  moments of the \textbf{returns} of the basket
%\item hermite tree by matching the first \textbf{four}  moments of the \textbf{returns} of the basket substituting binomial distribution with \textbf{normal} distribution
%\item hermite tree by matching   the first \textbf{four}  moments of the \textbf{value} of the basket substituting binomial distribution with normal distribution.
%\end{itemize}

The comparison was carried on the six baskets proposed in \cite{BorovkovaPermanaWeide2012} but considering as underlying stocks instead of futures. See table \ref{tab:baskets} for the details of the baskets. In the last row of that table, the distribution selected by \cite{BorovkovaPermanaWeide2007} is shown. Table  \ref{tab:result} shows the comparison with the method in \cite{BorovkovaPermanaWeide2007} The best method (excluding the brute Monte Carlo), considering as criterium the mean square error (MSE), is the \emph{H-6M-B-a}.

Some of the variants gave bad results  and for this reason they have been excluded from the comparison.


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]\footnotesize
  \centering
  \caption{Test baskets (\cite{BorovkovaPermanaWeide2012})}
    \begin{tabular}{|r|c|c|c|c|c|c|}
\cline{2-7}    \multicolumn{1}{r|}{} & Basket 1 & Basket 2 & Basket 3 & Basket 4 & Basket 5 & Basket 6 \\
    \hline
    Stock Prices & [100,120] & [150,100] & [110,90] & [200,50] & [95,90,105] & [100,90,95] \\
    \hline
    Volatility & [0.2,0.3] & [0.3,0.2] & [0.3,0.2] & [0.1,0.15] & [0.2,0.3,0.25] & [0.25,0.3,0.2] \\
    \hline
    Weights & [-1,1] & [-1,1] & [0.7,0.3] & [-1,1] & [1,-0.8,-0.5] & [0.6,0.8,-1] \\
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[2]{*}{Correlation}} & \multirow{2}[2]{*}{0.9} & \multirow{2}[2]{*}{0.3} & \multirow{2}[2]{*}{0.9} & \multirow{2}[2]{*}{0.8} & $\rho_{1,2}=\rho_{2,3}=0.9$,  & $\rho_{1,2}=\rho_{2,3}=0.9$,  \\
    \multicolumn{1}{|c|}{} &  &  &  &  & $\rho_{1,3}=0.8$ & $\rho_{1,3}=0.8$ \\
    \hline
    Strike price & 20 & -50 & 104 & -140 & -30 & 35 \\
    \hline
    Distribution & Shifted & Neg. shifted & Standard & Neg. shifted & Neg. shifted & Shifted \\
    \hline
    \end{tabular}%
  \label{tab:baskets}%
\end{table}%


\begin{table}[htbp]\footnotesize
  \centering
  \caption{Comparison between Monte Carlo with control variate prices and the other methods: Numerical Integration}
    \begin{tabular}{|r|r|r|r|r|r|r|}
    \hline
     & \multicolumn{6}{c|}{Prices}   \\
    \hline
     & \multicolumn{1}{c|}{MC-CV} & \multicolumn{1}{c|}{MC} & \multicolumn{1}{c|}{Borovkova} & \multicolumn{1}{c|}{H-4M-B-0} & \multicolumn{1}{c|}{H-4M-B-a} & \multicolumn{1}{c|}{H-6M-B-a}   \\
    \hline
    \multicolumn{1}{|c|}{Basket 1} & 8.2156(0.0062) & 8.2291(0.0148) & 8.24419433 & 8.6694 & 8.1916 & 8.2259   \\
    \hline
    \multicolumn{1}{|c|}{Basket 2} & 16.4512(0.0104) & 16.4608(0.0218) & 16.6215267 & 17.7485 & 16.4606 & 16.4912   \\
    \hline
    \multicolumn{1}{|c|}{Basket 3} & 12.5905(0.0011) & 12.5993(0.0204) & 12.5910619 & 12.5783 & 13.3633 & 12.5527   \\
    \hline
    \multicolumn{1}{|c|}{Basket 4} & 1.1461(0.0016) & 1.1481(0.0034) & 1.14555346 & 1.1451 & 1.1442 & 1.09   \\
    \hline
    \multicolumn{1}{|c|}{Basket 5} & 7.4794(0.0054) & 7.4821(0.0094) & 7.49507601 & 7.704 & 7.4574 & 7.4799   \\
    \hline
    \multicolumn{1}{|c|}{Basket 6} & 9.788(0.0061) & 9.7577(0.0158) & 9.7988865 & 9.9059 & 9.7387 & 9.7625   \\
    \hline
    \multicolumn{1}{|c|}{} & \multicolumn{6}{c|}{Absolute Errors}   \\
    \hline
    \multicolumn{1}{|c|}{Basket 1} & \multicolumn{1}{c|}{-} & 0.0136 & 0.0286 & 0.4538 & 0.024 & 0.0103   \\
    \hline
    \multicolumn{1}{|c|}{Basket 2} & \multicolumn{1}{c|}{-} & 0.0095 & 0.1703 & 1.2973 & 0.0094 & 0.04   \\
    \hline
    \multicolumn{1}{|c|}{Basket 3} & \multicolumn{1}{c|}{-} & 0.0088 & \textbf{0.0006} & 0.0122 & 0.7728 & 0.0378   \\
    \hline
    \multicolumn{1}{|c|}{Basket 4} & \multicolumn{1}{c|}{-} & 0.002 & 0.0005 & 0.001 & 0.0019 & 0.0561   \\
    \hline
    \multicolumn{1}{|c|}{Basket 5} & \multicolumn{1}{c|}{-} & 0.0027 & 0.0156 & 0.2246 & 0.022 & \textbf{0.0005}   \\
    \hline
    \multicolumn{1}{|c|}{Basket 6} & \multicolumn{1}{c|}{-} & 0.0303 & 0.0109 & 0.1179 & 0.0493 & 0.0255   \\
    \hline
    \multicolumn{1}{|c|}{MSE} & \multicolumn{1}{c|}{-} & 0.000214 & 0.00503047 & 0.325569523 & 0.10013372 & 0.00115544   \\
    \hline
    \multicolumn{1}{|c|}{} & \multicolumn{6}{c|}{Prices}   \\
    \hline
    \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{H-4M-B-b} & \multicolumn{1}{c|}{H-6M-B-b} & \multicolumn{1}{c|}{H-4M-N-a} & \multicolumn{1}{c|}{H-6M-N-a} & \multicolumn{1}{c|}{H-4M-N-b} & \multicolumn{1}{c|}{H-6M-N-b}   \\
    \hline
    \multicolumn{1}{|c|}{Basket 1} & 8.1916 & 8.2259 & 8.1977 & 8.2224 & 8.1977 & 8.2224   \\
    \hline
    \multicolumn{1}{|c|}{Basket 2} & 16.4606 & 16.4912 & 16.4424 & 16.4634 & 16.4424 & 16.4633   \\
    \hline
    \multicolumn{1}{|c|}{Basket 3} & 12.5559 & 12.5796 & 13.3451 & 13.4526 & 12.5698 & 12.5891   \\
    \hline
    \multicolumn{1}{|c|}{Basket 4} & 1.1454 & 1.12 & 1.145 & 1.1661 & 1.1457 & 1.1457   \\
    \hline
    \multicolumn{1}{|c|}{Basket 5} & 7.4574 & 7.4799 & 7.4564 & 7.4721 & 7.4563 & 7.4721   \\
    \hline
    \multicolumn{1}{|c|}{Basket 6} & 9.7387 & 9.7745 & 9.7625 & 9.7822 & 9.7628 & 9.7821   \\
    \hline
    \multicolumn{1}{|c|}{} & \multicolumn{6}{c|}{Absolute Errors}   \\
    \hline
    \multicolumn{1}{|c|}{Basket 1} & 0.024 & 0.0103 & 0.0179 & \textbf{0.0068} & \textbf{0.0179} & \textbf{0.0068}   \\
    \hline
    \multicolumn{1}{|c|}{Basket 2} & 0.0094 & 0.04 & \textbf{0.0088} & 0.0122 & \textbf{0.0088} & 0.0121   \\
    \hline
    \multicolumn{1}{|c|}{Basket 3} & 0.0346 & 0.0109 & 0.7546 & 0.8621 & 0.0207 & 0.0014   \\
    \hline
    \multicolumn{1}{|c|}{Basket 4} & 0.0007 & 0.0261 & 0.0011 & 0.02 & \textbf{0.0004} & \textbf{0.0004}   \\
    \hline
    \multicolumn{1}{|c|}{Basket 5} & 0.022 & \textbf{0.0005} & 0.023 & 0.0073 & 0.0231 & 0.0073   \\
    \hline
    \multicolumn{1}{|c|}{Basket 6} & 0.0493 & 0.0135 & 0.0255 & \textbf{0.0058} & 0.0252 & 0.0059   \\
    \hline
    \multicolumn{1}{|c|}{MSE} & 0.000796083 & 0.000448102 & 0.09516658 & 0.12398307 & \textbf{0.00033253} & \textbf{0.000047145}   \\
    \hline
    \end{tabular}\\
      \label{tab:result}%
        Data for the baskets are described in \cite{BorovkovaPermanaWeide2012} with $T=1$, $r=3\%$, $\delta=0$. In the first part of the table (``Prices'') are reported the prices of each options using the different methods. In the second part, each method is compared with the Monte Carlo method with control variates.
\end{table}%

\newpage
\subsection{More robust comparison}
The comparison is carried considering $\#$ randomly generated instances. In particular, the parameters where selected to be the same of \cite{BroadieEtAl1994}:
\begin{itemize}
\item risk free rate equal to 0 with probability 0.0 and uniformly distributed between 0.0 and 0.1 with probability 0.8.
\item volatility uniformly distributed between 0.1 and 0.6.
\item time-to-maturity uniformly distributed between 0.1 and 1 years with probability 0.75 and between 1 and 5 years with probability 0.25
\item spot prices uniformly distributed between 70 and 130.
\end{itemize}
Furthermore, the other parameters are:
\begin{itemize}
\item weights of assets in the basket uniformly distributed between -1 and 1
\item for each instances three different strike prices are considered. One that makes the option at-the-money, two randomly selected to  have an in-the-money option and an out-of-the-money option. The randomness consists of a variation in a range of 30 dollars respectively up and down the at-the-money strike)
\item the correlation matrix randomly generated satisfying the semi-positiveness condition (see for example \cite{RousseeuwMolenberghs1994})
\end{itemize} 

==> shiftedHermiteMethod.tex <==

The standard Hermite tree method for some baskets has poor performances that mainly derive from the difficulties to match the moments of the basket. A solution to this problem is the shifting of the basket by a parameter $\tau$ so that the matching of the moments is carried between the moments of the Hermite function and the moments of the shifted basket. This method appears like the method in \cite{BorovkovaPermanaWeide2012} given the parameter $\tau$ but it is different from that because the shift here is in the basket while the latter shifts the standard log-normal density probability.
The performances of the shifted Hermite tree method depend on the selection of the shift, $\tau$. In the following, three different ways to find the "right" $\tau$ are proposed. Firstly, $\tau$ can be calculated by using the method in \cite{BorovkovaPermanaWeide2012} assuming that the shift for the basket has the same value of the shift that allows the match of moments in \cite{BorovkovaPermanaWeide2012} (see results in table \ref{tab:Shift04M}).
% Table generated by Excel2LaTeX from sheet 'Shift'
\begin{table}[htbp]
  \centering
  \caption{Prices and Error (compared to Monte carlo method with control variate) using the shifted Hermite tree with the shift given by Borovkova formula}
    \begin{tabular}{|r|r|r|}
\cline{2-3}    \multicolumn{1}{r|}{} & \multicolumn{2}{c|}{Shifted-H-$(m+1)$M-B-0} \\
    \hline
    \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{Price} & \multicolumn{1}{c|}{Error} \\
    \hline
    Basket 1 & 8.243044521 & 0.013908189 \\
    \hline
    Basket 2 & 17.96965069 & 1.508872524 \\
    \hline
    Basket 3 & 12.57892479 & 0.020375967 \\
    \hline
    Basket 4 & 1.145147659 & 0.002955167 \\
    \hline
    Basket 5 & 6.195737309 & 0.080096712 \\
    \hline
    Basket 6 & 10.00643906 & 0.013652466 \\
    \hline
    \multicolumn{2}{|c|}{MSE} & 0.380652587 \\
    \hline
    \end{tabular}%
  \label{tab:Shift04M}%
\end{table}%

Secondly, it is possible to consider one extra moment (the $m+1$-th one) to match $\tau$ as explained below. Considering the variant H-$(m+1)$M-B-0 with shift, the matching of moments consists in the solution of the non-linear system of equation:
\begin{equation}
\esp\left[\left(\frac{B(T)-\tau}{ B(0)\ee^{rT}}\right)^k\right]=\sum_{i=0}^{k}{\binom{k}{i}\frac{(-\tau)^i}{(B(0)\ee^{rt})^{k}}\esp[B^{k-i}(t)]}=Y'^k \cdot P.
\end{equation}
There are $m+2$ unknowns ($\lambda_0,\ldots,\lambda_m$ and $\tau$) so the first $m+2$ moments have to be considered.
Finally, an iterative algorithm to find the "best"\footnote{ The "best" is the $\tau$ that allows the match of the moments with the smallest error.}  $\tau$ is proposed:
\begin{enumerate}
\item Select a $\tau$ (how to select tau is explained below)
\item Calculate the parameters $\lambda_0,\ldots,\lambda_m$ and the error between the real moments and the moments for the parameters calculated\footnote{It should be notice that the parameter calculated for one $\tau$ can be used as initial solution for the solution of the system for the next system}.
\item If the error in step 2 is smaller than the best found, select it as the best one, otherwise, go to step 1.
\end{enumerate}
The selection of $\tau$ can be done incrementally or randomly but the range within it is searched becomes really important to have good performance. From empirically studies it results that the  shift to be selected is the one that moves $B(0)$, the current value of the basket, far from zero. The methods above should help to understand how far from zero and with direction should be taken (either the positive direction or the negative one).
